Global Average Precision for Representation Learning

Standard information retrieval metrics, such as mean Average Precision (mAP), assess performance one query at a time, based on how the similarities between a query and its positives compare against those with its negatives. The same holds for common representation learning losses, such as InfoNCE and per-query AP surrogates. None of them considers whether similarities are comparable across queries, which any system with a single decision threshold relies on. Global Average Precision (gAP) does, by ranking all query-candidate pairs in one list and computing a single AP. We introduce gSAP, a differentiable surrogate of gAP. It needs only a similarity matrix and a binary matrix marking the positive pairs, the same input as existing losses, so it is a drop-in replacement for them and agnostic to the encoder, the modality, and the source of supervision. Since it considers all possible pairwise comparisons in the batch jointly, it also remains trainable at low temperatures, a regime where per-query surrogates run out of gradient. Swapping it into established recipes improves supervised metric learning, cross-modal alignment, and self-supervised pretraining, where, to our knowledge, it is the first ranking loss to replace the community standard InfoNCE in the latter two. Its similarities are more consistent across queries, which drives the gains under a universal threshold. gSAP retrieves up to four times as many positive pairs as the strongest AP surrogate at the same precision, and it degrades the least when queries with no positives in the database are added. Beyond thresholding, models trained with gSAP also learn better representations, with higher transfer, $k$NN and zero-shot classification accuracy.

==> data/dino_map.tex <==
\pgfplotstableread{
percentage	SAP_2	SAP_4	SGAP_2	SGAP_4	RecK_2	RecK_4
1	43.45	46.20	46.35	51.79	42.83	50.90
5	54.38	59.60	55.37	59.22	54.26	59.13
10	57.53	62.58	59.92	63.61	58.64	62.79
25	62.70	66.72	63.45	66.41	61.91	66.14
50	65.31	68.22	65.79	69.24	64.84	68.51
100	68.18	71.24	67.74	71.59	67.41	70.77
}{\sop}

\pgfplotstableread{
percentage	SAP_2	SAP_4	SGAP_2	SGAP_4	RecK_2	RecK_4
1	27.44	30.16	29.20	31.18	29.04	30.48
5	30.80	32.72	32.23	33.17	31.19	32.42
10	31.24	33.98	31.99	34.65	31.27	34.34
25	34.53	36.44	33.58	35.31	33.37	36.60
50	36.18	38.39	35.81	38.61	34.91	37.86
100	37.20	40.19	37.53	40.70	36.21	39.82
}{\inat}

\pgfplotstableread{
percentage	SAP_2	SAP_3	SAP_4	SAP_5	SGAP_2	SGAP_3	SGAP_4	SGAP_5	RecK_2	RecK_3	RecK_4	RecK_5
1	39.76	43.22	45.75	46.21	40.70	45.11	45.98	47.64	40.06	43.10	45.00	46.26
5	44.06	55.04	55.82	56.32	51.61	55.73	56.21	57.19	49.82	53.95	56.09	56.41
10	53.29	58.12	59.59	59.72	55.95	58.84	59.72	60.04	54.77	57.72	59.29	59.65
25	58.08	61.62	63.21	63.66	60.14	62.48	63.17	63.73	58.76	61.25	62.55	63.22
50	65.60	66.68	66.07	66.23	63.07	65.10	66.04	66.31	61.76	64.16	65.12	65.42
100	65.16	67.72	68.48	68.77	65.60	67.48	68.59	68.08	64.50	66.84	67.77	67.76
}{\sopv}

\pgfplotstableread{
percentage	SAP_2	SAP_3	SAP_4	SAP_5	SGAP_2	SGAP_3	SGAP_4	SGAP_5	RecK_2	RecK_3	RecK_4	RecK_5
1	23.94	29.48	30.08	31.42	25.90	30.15	30.84	31.42	25.05	28.61	30.57	30.54
5	29.05	33.35	34.51	34.60	32.44	33.85	35.45	34.95	31.90	32.42	34.12	34.67
10	32.54	33.46	35.26	35.82	34.36	35.42	35.73	36.23	33.60	34.54	35.37	35.53
25	35.29	36.63	37.74	38.22	35.88	37.72	37.97	38.20	34.24	35.67	37.51	37.15
50	35.87	37.85	39.57	40.16	37.27	39.11	39.80	39.57	35.33	38.03	39.25	39.69
100	39.26	40.25	42.08	42.64	39.16	40.76	41.33	42.55	37.61	40.36	41.49	41.80
}{\inatv}

\pgfplotstableread{
percentage	SAP_2	SAP_3	SAP_4	SAP_5	SGAP_2	SGAP_3	SGAP_4	SGAP_5	RecK_2	RecK_3	RecK_4	RecK_5
5	2.53	5.40	8.08	9.96	2.29	5.68	10.00	10.25	1.52	3.98	9.33	9.57
10	6.96	9.94	15.71	18.93	10.77	15.40	16.71	21.56	6.25	13.30	16.32	20.27
25	10.59	22.07	27.67	29.36	14.72	25.81	28.22	31.70	19.02	23.17	25.89	29.94
50	21.81	27.17	31.18	36.33	22.44	31.86	34.60	36.22	22.11	30.71	34.18	36.70
100	25.86	33.78	37.29	35.34	25.75	34.48	37.93	37.70	27.85	34.31	39.51	40.86
}{\cars}


==> data/dino_uap.tex <==
\pgfplotstableread{
percentage	SAP_2	SAP_4	SGAP_2	SGAP_4	RecK_2	RecK_4
1	14.99	17.20	20.68	23.25	15.74	20.76
5	27.89	37.80	35.60	39.15	28.76	37.25
10	34.92	41.78	41.02	45.06	35.14	42.24
25	42.85	47.77	46.36	49.23	41.67	46.98
50	46.95	50.18	50.50	53.63	45.68	50.54
100	51.82	54.97	53.84	57.25	50.35	53.98
}{\sop}

\pgfplotstableread{
percentage	SAP_2	SAP_4	SGAP_2	SGAP_4	RecK_2	RecK_4
1	9.11	10.38	11.75	12.29	8.21	10.11
5	12.11	13.42	14.89	16.20	12.62	13.35
10	13.13	15.18	16.06	18.49	12.43	15.61
25	16.19	18.76	19.27	20.68	15.74	18.61
50	18.78	20.89	21.95	24.12	16.90	20.69
100	20.35	23.76	23.85	26.76	19.50	23.17
}{\inat}

\pgfplotstableread{
percentage	SAP_2	SAP_3	SAP_4	SAP_5	SGAP_2	SGAP_3	SGAP_4	SGAP_5	RecK_2	RecK_3	RecK_4	RecK_5
1	13.55	16.00	17.03	17.65	14.42	16.34	17.57	19.07	12.67	14.40	17.25	17.89
5	23.42	32.59	34.08	34.80	31.95	36.37	35.83	37.05	26.10	31.72	33.21	34.14
10	31.72	37.25	38.32	38.37	37.30	40.15	40.45	40.43	32.83	36.99	38.02	38.00
25	37.50	41.72	42.40	43.48	43.42	44.71	44.40	45.22	38.34	40.87	41.85	42.72
50	46.80	48.03	47.14	47.31	47.01	48.82	49.25	49.49	42.37	45.49	45.93	46.27
100	48.17	50.60	51.19	51.05	50.83	52.35	53.07	52.19	46.26	49.23	49.90	50.25
}{\sopv}

\pgfplotstableread{
percentage	SAP_2	SAP_3	SAP_4	SAP_5	SGAP_2	SGAP_3	SGAP_4	SGAP_5	RecK_2	RecK_3	RecK_4	RecK_5
1	5.85	7.94	8.87	8.93	7.38	9.90	10.38	9.91	6.44	7.01	8.39	8.30
5	10.26	11.89	13.02	13.64	16.32	16.53	18.25	16.97	10.24	10.29	12.91	13.51
10	14.13	16.05	16.23	16.65	18.99	19.72	19.46	19.54	13.47	16.30	16.43	16.33
25	18.17	18.94	20.29	20.36	21.09	22.11	22.33	22.25	17.21	18.47	19.80	19.62
50	19.42	20.94	22.27	22.65	23.16	24.29	24.58	24.11	18.93	20.83	21.48	22.07
100	21.99	23.55	24.62	24.69	25.72	26.54	26.83	27.46	20.45	22.84	23.63	23.63
}{\inatv}

\pgfplotstableread{
percentage	SAP_2	SAP_3	SAP_4	SAP_5	SGAP_2	SGAP_3	SGAP_4	SGAP_5	RecK_2	RecK_3	RecK_4	RecK_5
5	1.56	3.15	4.67	5.17	1.43	3.71	5.15	5.35	1.18	2.69	4.91	4.68
10	4.45	6.14	10.11	12.52	7.21	9.75	11.49	13.85	3.73	7.74	10.07	13.31
25	7.09	15.10	19.85	21.53	9.33	18.96	20.84	23.77	12.41	16.29	18.02	21.20
50	14.95	20.21	23.32	27.20	17.47	25.08	27.17	29.23	15.54	22.68	25.39	27.85
100	18.72	26.25	28.96	27.38	20.25	27.92	31.49	31.11	20.55	26.04	31.01	31.98
}{\carsv}


==> data/loss_comparison_v2.tex <==
\pgfplotstableread{
iteration SAP_loss SAP_mAP SAP_uAP SAP_gnorm SAP_unsat SAP_eff SAP_unsatpp SGAP_loss SGAP_mAP SGAP_uAP SGAP_gnorm SGAP_unsat SGAP_eff SGAP_unsatpp
0 14.44 51.92 32.57 4.8463e-02 5.0047e+01 2.3227e+01 4.9947e+02 7.14 51.92 32.57 3.0212e-02 4.9532e+01 2.2859e+01 4.9483e+05
1 16.62 53.91 35.86 5.2233e-02 4.7377e+01 2.2020e+01 4.7282e+02 8.61 54.31 36.69 3.5965e-02 4.6625e+01 2.1515e+01 4.6578e+05
2 18.58 55.53 39.20 5.5005e-02 4.5219e+01 2.1001e+01 4.5128e+02 10.10 56.46 40.94 4.1434e-02 4.4215e+01 2.0354e+01 4.4171e+05
3 20.46 57.17 42.12 5.7119e-02 4.3346e+01 2.0133e+01 4.3260e+02 11.64 58.50 44.60 4.6606e-02 4.2156e+01 1.9354e+01 4.2113e+05
4 22.20 58.55 45.11 5.8953e-02 4.1799e+01 1.9383e+01 4.1715e+02 13.15 60.10 48.04 5.1306e-02 4.0444e+01 1.8519e+01 4.0404e+05
5 23.81 59.79 47.74 6.0239e-02 4.0436e+01 1.8742e+01 4.0355e+02 14.62 61.73 50.94 5.5457e-02 3.8947e+01 1.7790e+01 3.8908e+05
6 25.58 61.10 50.81 6.1625e-02 3.8914e+01 1.7826e+01 3.8836e+02 16.33 63.54 54.18 5.9934e-02 3.7335e+01 1.6829e+01 3.7297e+05
7 27.18 62.38 53.12 6.2407e-02 3.7736e+01 1.7215e+01 3.7661e+02 17.93 65.07 56.55 6.3781e-02 3.6092e+01 1.6184e+01 3.6056e+05
8 28.78 63.85 55.54 6.3217e-02 3.6375e+01 1.6496e+01 3.6302e+02 19.60 66.67 58.92 6.7311e-02 3.4670e+01 1.5468e+01 3.4635e+05
9 30.31 64.80 57.59 6.3878e-02 3.5200e+01 1.5884e+01 3.5129e+02 21.23 67.83 60.86 7.0396e-02 3.3474e+01 1.4868e+01 3.3441e+05
10 31.97 66.18 59.67 6.4387e-02 3.3918e+01 1.5209e+01 3.3850e+02 23.06 69.38 62.81 7.3418e-02 3.2145e+01 1.4225e+01 3.2113e+05
11 33.37 67.14 61.34 6.4982e-02 3.2921e+01 1.4726e+01 3.2855e+02 24.66 70.34 64.37 7.5800e-02 3.1186e+01 1.3780e+01 3.1155e+05
12 34.79 68.26 62.86 6.5186e-02 3.1922e+01 1.4282e+01 3.1858e+02 26.32 71.63 65.80 7.7847e-02 3.0155e+01 1.3350e+01 3.0125e+05
13 36.21 69.50 64.47 6.5488e-02 3.0778e+01 1.3739e+01 3.0716e+02 27.99 72.78 67.33 7.9701e-02 2.9062e+01 1.2868e+01 2.9033e+05
14 37.58 70.45 65.96 6.5839e-02 2.9850e+01 1.3295e+01 2.9790e+02 29.69 73.77 68.75 8.1411e-02 2.8175e+01 1.2501e+01 2.8147e+05
15 39.03 71.59 67.29 6.5946e-02 2.8861e+01 1.2852e+01 2.8803e+02 31.43 74.79 70.05 8.2852e-02 2.7264e+01 1.2136e+01 2.7237e+05
16 40.49 72.63 68.49 6.5966e-02 2.7993e+01 1.2524e+01 2.7937e+02 33.25 75.63 71.24 8.4051e-02 2.6479e+01 1.1845e+01 2.6453e+05
17 41.82 73.36 69.79 6.6172e-02 2.7059e+01 1.2061e+01 2.7005e+02 34.92 76.56 72.50 8.4980e-02 2.5637e+01 1.1419e+01 2.5611e+05
18 43.38 74.73 71.21 6.6251e-02 2.6050e+01 1.1637e+01 2.5998e+02 36.88 77.74 73.82 8.5836e-02 2.4772e+01 1.1073e+01 2.4747e+05
19 44.76 75.55 72.36 6.6383e-02 2.5236e+01 1.1317e+01 2.5185e+02 38.62 78.77 74.98 8.6333e-02 2.3982e+01 1.0794e+01 2.3958e+05
20 46.06 76.29 73.50 6.6497e-02 2.4498e+01 1.1010e+01 2.4449e+02 40.31 79.41 76.07 8.6665e-02 2.3334e+01 1.0555e+01 2.3310e+05
}{\spcfourtauone}

\pgfplotstableread{
iteration SAP_loss SAP_mAP SAP_uAP SAP_gnorm SAP_unsat SAP_eff SAP_unsatpp SGAP_loss SGAP_mAP SGAP_uAP SGAP_gnorm SGAP_unsat SGAP_eff SGAP_unsatpp
0 51.13 51.92 32.57 1.1101e-01 3.9836e+00 1.9815e+00 3.9756e+01 32.28 51.92 32.57 2.1208e-01 3.9161e+00 1.9523e+00 3.9122e+04
1 55.57 56.36 36.56 1.0269e-01 3.5918e+00 1.7870e+00 3.5846e+01 39.90 54.41 40.33 1.7069e-01 3.7119e+00 1.8504e+00 3.7082e+04
2 59.33 60.03 41.14 1.0153e-01 3.2345e+00 1.6115e+00 3.2281e+01 45.97 57.01 46.43 1.4860e-01 3.5191e+00 1.7541e+00 3.5156e+04
3 62.62 63.17 45.34 9.4120e-02 2.8950e+00 1.4427e+00 2.8892e+01 50.89 59.63 51.39 1.3850e-01 3.3121e+00 1.6507e+00 3.3088e+04
4 65.50 66.16 49.62 9.8290e-02 2.6495e+00 1.3208e+00 2.6442e+01 55.27 62.09 55.78 1.3264e-01 3.1206e+00 1.5552e+00 3.1174e+04
5 67.96 68.71 53.17 9.4830e-02 2.4441e+00 1.2171e+00 2.4392e+01 58.93 64.53 59.46 1.2717e-01 2.9620e+00 1.4757e+00 2.9590e+04
6 70.54 71.29 57.39 9.4748e-02 2.2021e+00 1.0972e+00 2.1977e+01 62.87 67.42 63.38 1.1985e-01 2.7427e+00 1.3663e+00 2.7399e+04
7 72.73 73.31 60.70 8.7917e-02 2.0604e+00 1.0268e+00 2.0563e+01 66.01 69.81 66.50 1.1311e-01 2.5993e+00 1.2946e+00 2.5967e+04
8 74.74 75.24 63.97 8.7202e-02 1.8819e+00 9.3444e-01 1.8782e+01 68.90 71.79 69.37 1.0658e-01 2.4342e+00 1.2119e+00 2.4317e+04
9 76.81 77.35 66.94 8.5871e-02 1.7603e+00 8.7231e-01 1.7568e+01 71.61 74.10 72.08 1.0340e-01 2.2840e+00 1.1371e+00 2.2817e+04
10 78.69 79.22 69.72 8.6837e-02 1.6355e+00 8.1582e-01 1.6323e+01 74.14 76.09 74.58 9.8527e-02 2.1363e+00 1.0636e+00 2.1342e+04
11 80.37 80.87 72.05 8.3346e-02 1.5435e+00 7.6735e-01 1.5404e+01 76.25 77.84 76.67 9.3445e-02 2.0323e+00 1.0113e+00 2.0303e+04
12 81.77 82.25 74.12 7.8083e-02 1.4637e+00 7.2788e-01 1.4608e+01 78.18 79.59 78.57 8.6610e-02 1.9190e+00 9.5490e-01 1.9171e+04
13 83.20 83.61 76.14 7.6799e-02 1.3857e+00 6.8605e-01 1.3829e+01 79.89 81.09 80.24 7.8793e-02 1.8226e+00 9.0753e-01 1.8208e+04
14 84.50 84.85 78.10 7.0018e-02 1.3114e+00 6.5188e-01 1.3088e+01 81.27 82.39 81.58 7.5889e-02 1.7240e+00 8.5817e-01 1.7222e+04
15 85.64 85.93 79.69 6.4379e-02 1.2691e+00 6.2906e-01 1.2666e+01 82.62 83.62 82.91 7.3265e-02 1.6565e+00 8.2473e-01 1.6548e+04
16 86.70 87.02 81.28 6.6735e-02 1.2065e+00 6.0314e-01 1.2041e+01 83.91 84.79 84.18 7.1446e-02 1.5645e+00 7.7924e-01 1.5630e+04
17 87.78 88.10 82.70 6.0750e-02 1.1349e+00 5.6353e-01 1.1326e+01 85.15 85.88 85.41 7.1150e-02 1.4734e+00 7.3394e-01 1.4719e+04
18 88.81 89.08 84.33 5.8683e-02 1.0927e+00 5.4403e-01 1.0905e+01 86.34 86.92 86.58 7.1008e-02 1.4261e+00 7.1086e-01 1.4246e+04
19 89.64 89.89 85.53 5.9202e-02 1.0457e+00 5.2163e-01 1.0436e+01 87.62 88.21 87.86 6.7794e-02 1.3388e+00 6.6748e-01 1.3375e+04
20 90.48 90.73 86.68 5.6936e-02 9.9018e-01 4.9597e-01 9.8820e+00 88.64 89.12 88.87 6.1578e-02 1.2821e+00 6.3930e-01 1.2809e+04
}{\spcfourtautwo}

\pgfplotstableread{
iteration SAP_loss SAP_mAP SAP_uAP SAP_gnorm SAP_unsat SAP_eff SAP_unsatpp SGAP_loss SGAP_mAP SGAP_uAP SGAP_gnorm SGAP_unsat SGAP_eff SGAP_unsatpp
0 51.89 51.92 32.57 2.2828e-01 4.0207e-01 2.0174e-01 4.0127e+00 32.55 51.92 32.57 2.1795e-01 3.8865e-01 1.9430e-01 3.8826e+03
1 54.57 54.59 35.01 2.2017e-01 3.6630e-01 1.8391e-01 3.6557e+00 40.23 54.31 40.24 2.0878e-01 3.6849e-01 1.8419e-01 3.6812e+03
2 57.13 57.18 38.01 2.2728e-01 3.3988e-01 1.6952e-01 3.3920e+00 46.33 56.96 46.34 1.5033e-01 3.4894e-01 1.7463e-01 3.4859e+03
3 59.22 59.25 40.57 2.5385e-01 3.1323e-01 1.5722e-01 3.1260e+00 51.30 59.61 51.31 1.3900e-01 3.2867e-01 1.6438e-01 3.2834e+03
4 61.23 61.27 43.58 2.2319e-01 2.9426e-01 1.4808e-01 2.9367e+00 55.70 61.99 55.71 1.3388e-01 3.1022e-01 1.5520e-01 3.0991e+03
5 62.91 62.94 45.97 2.0681e-01 2.8126e-01 1.4104e-01 2.8070e+00 59.32 64.46 59.32 1.2959e-01 2.9431e-01 1.4716e-01 2.9402e+03
6 64.95 65.02 49.08 2.4917e-01 2.6179e-01 1.3126e-01 2.6127e+00 63.31 67.36 63.31 1.2198e-01 2.7164e-01 1.3587e-01 2.7137e+03
7 66.64 66.68 51.56 1.9988e-01 2.5281e-01 1.2715e-01 2.5230e+00 66.42 69.69 66.42 1.1494e-01 2.5735e-01 1.2878e-01 2.5710e+03
8 68.31 68.34 54.21 1.9431e-01 2.3591e-01 1.1824e-01 2.3543e+00 69.29 71.78 69.29 1.0819e-01 2.4042e-01 1.2031e-01 2.4018e+03
9 69.83 69.87 56.61 1.9839e-01 2.2605e-01 1.1374e-01 2.2560e+00 71.98 74.00 71.98 1.0577e-01 2.2595e-01 1.1308e-01 2.2572e+03
10 71.40 71.43 58.85 2.0222e-01 2.1687e-01 1.0873e-01 2.1643e+00 74.48 75.96 74.49 1.0123e-01 2.1112e-01 1.0564e-01 2.1091e+03
11 72.76 72.79 60.86 2.1846e-01 2.0578e-01 1.0200e-01 2.0537e+00 76.66 77.82 76.66 9.5023e-02 1.9899e-01 9.9547e-02 1.9879e+03
12 73.96 73.99 62.64 2.0560e-01 1.9927e-01 9.9160e-02 1.9887e+00 78.57 79.67 78.58 8.8607e-02 1.8839e-01 9.4234e-02 1.8820e+03
13 75.27 75.30 64.29 2.2838e-01 1.8975e-01 9.4888e-02 1.8937e+00 80.25 81.12 80.26 8.0320e-02 1.7987e-01 8.9979e-02 1.7969e+03
14 76.63 76.69 65.99 1.8377e-01 1.7919e-01 8.9753e-02 1.7883e+00 81.62 82.40 81.62 7.7452e-02 1.7019e-01 8.5064e-02 1.7002e+03
15 77.61 77.67 67.35 2.3333e-01 1.6690e-01 8.3982e-02 1.6657e+00 82.95 83.55 82.96 7.5900e-02 1.6522e-01 8.2695e-02 1.6505e+03
16 78.64 78.66 68.75 1.7950e-01 1.6483e-01 8.2330e-02 1.6450e+00 84.21 84.76 84.22 7.1659e-02 1.5711e-01 7.8599e-02 1.5696e+03
17 79.63 79.64 70.10 1.5564e-01 1.5418e-01 7.8152e-02 1.5387e+00 85.34 85.76 85.34 7.0742e-02 1.4773e-01 7.3938e-02 1.4758e+03
18 80.77 80.83 71.87 2.2028e-01 1.5287e-01 7.6716e-02 1.5257e+00 86.54 86.89 86.54 7.2525e-02 1.4225e-01 7.1107e-02 1.4211e+03
19 81.63 81.66 73.17 2.2616e-01 1.4906e-01 7.4368e-02 1.4877e+00 87.77 88.03 87.78 6.9449e-02 1.3589e-01 6.8051e-02 1.3576e+03
20 82.46 82.51 74.26 1.6579e-01 1.4542e-01 7.3144e-02 1.4513e+00 88.71 88.73 88.72 6.3122e-02 1.3255e-01 6.6313e-02 1.3242e+03
}{\spcfourtauthree}

\pgfplotstableread{
iteration SAP_loss SAP_mAP SAP_uAP SAP_gnorm SAP_unsat SAP_eff SAP_unsatpp SGAP_loss SGAP_mAP SGAP_uAP SGAP_gnorm SGAP_unsat SGAP_eff SGAP_unsatpp
0 51.92 51.92 32.57 7.1644e-01 4.0848e-02 2.0941e-02 4.0767e-01 32.55 51.92 32.57 2.4084e-01 3.8983e-02 1.9551e-02 3.8944e+02
1 52.93 52.94 33.43 9.3517e-01 3.6573e-02 1.8511e-02 3.6500e-01 39.86 54.11 39.87 2.0731e-01 3.7087e-02 1.8605e-02 3.7050e+02
2 54.00 54.03 34.59 1.4356e+00 3.6373e-02 1.8549e-02 3.6300e-01 45.62 56.58 45.63 1.5511e-01 3.5358e-02 1.7738e-02 3.5322e+02
3 54.84 54.84 35.05 6.2006e-01 3.5003e-02 1.7291e-02 3.4933e-01 50.26 59.02 50.26 1.5643e-01 3.3408e-02 1.6745e-02 3.3375e+02
4 55.48 55.48 36.03 3.7155e-01 3.5237e-02 1.7867e-02 3.5167e-01 54.46 61.45 54.47 1.6326e-01 3.1720e-02 1.5911e-02 3.1688e+02
5 56.04 56.06 36.61 1.0317e+00 3.5605e-02 1.8288e-02 3.5533e-01 57.88 63.74 57.89 1.7426e-01 3.0270e-02 1.5190e-02 3.0240e+02
6 56.84 56.84 37.45 5.2170e-01 3.6740e-02 1.8593e-02 3.6667e-01 61.69 66.21 61.69 1.6172e-01 2.8290e-02 1.4214e-02 2.8262e+02
7 57.31 57.31 37.48 5.8331e-01 3.5037e-02 1.7829e-02 3.4967e-01 64.74 68.49 64.74 1.4265e-01 2.6748e-02 1.3428e-02 2.6721e+02
8 57.71 57.71 38.09 4.8303e-01 3.5137e-02 1.6685e-02 3.5067e-01 67.57 70.56 67.57 1.1465e-01 2.5126e-02 1.2644e-02 2.5101e+02
9 57.92 57.92 38.52 4.7227e-01 3.4168e-02 1.7278e-02 3.4100e-01 70.20 72.72 70.20 1.1317e-01 2.3403e-02 1.1761e-02 2.3380e+02
10 58.46 58.47 39.12 1.0855e+00 3.4836e-02 1.7292e-02 3.4767e-01 72.63 74.67 72.63 1.1420e-01 2.2058e-02 1.1082e-02 2.2036e+02
11 58.65 58.65 39.64 6.5895e-01 3.1630e-02 1.5681e-02 3.1567e-01 74.68 76.36 74.68 1.1071e-01 2.0889e-02 1.0521e-02 2.0868e+02
12 59.16 59.16 40.22 3.5197e-01 3.4569e-02 1.7504e-02 3.4500e-01 76.65 77.94 76.66 1.0767e-01 1.9856e-02 9.9652e-03 1.9836e+02
13 59.64 59.64 41.02 6.7038e-01 3.2999e-02 1.6349e-02 3.2933e-01 78.57 79.58 78.57 9.8733e-02 1.8845e-02 9.4735e-03 1.8826e+02
14 60.35 60.35 42.38 6.5387e-01 3.1430e-02 1.5604e-02 3.1367e-01 80.08 80.97 80.08 8.7095e-02 1.7932e-02 9.0061e-03 1.7915e+02
15 61.02 61.02 43.10 3.8900e-01 3.1764e-02 1.5794e-02 3.1700e-01 81.37 82.14 81.37 8.9382e-02 1.7418e-02 8.7562e-03 1.7400e+02
16 61.71 61.71 43.87 6.1312e-01 2.9993e-02 1.5240e-02 2.9933e-01 82.63 83.29 82.63 8.0240e-02 1.6626e-02 8.3653e-03 1.6609e+02
17 62.11 62.12 44.74 1.0586e+00 3.1396e-02 1.5601e-02 3.1333e-01 83.83 84.40 83.83 8.2363e-02 1.5650e-02 7.8925e-03 1.5635e+02
18 62.94 62.94 46.03 3.8501e-01 2.6653e-02 1.3491e-02 2.6600e-01 85.06 85.61 85.06 7.9491e-02 1.5313e-02 7.6740e-03 1.5297e+02
19 63.62 63.62 47.06 5.6566e-01 2.8390e-02 1.3749e-02 2.8333e-01 86.26 86.74 86.26 7.6637e-02 1.4368e-02 7.2101e-03 1.4354e+02
20 64.07 64.07 47.51 4.6228e-01 2.8257e-02 1.4651e-02 2.8200e-01 87.31 87.64 87.31 7.5522e-02 1.3570e-02 6.8418e-03 1.3556e+02
}{\spcfourtaufour}



==> data/sim_dist_data.tex <==
\pgfplotstableread{
sim dist
0.4183381 0.0
0.43850538 0.0
0.45867267 0.0
0.47883996 4.0
0.49900728 0.0
0.5191746 0.0
0.53934187 0.0
0.55950916 4.0
0.57967645 16.0
0.59984374 48.0
0.62001103 56.0
0.6401783 80.0
0.6603456 62.0
0.6805129 58.0
0.7006802 72.0
0.7208475 44.0
0.74101484 36.0
0.7611821 34.0
0.7813494 18.0
0.8015167 6.0
0.821684 10.0
0.8418513 2.0
0.8620186 0.0
0.8821859 2.0
0.883 0.0
}{\sgappos}

\pgfplotstableread{
sim dist
0.40 0.0
0.4544161 91.0
0.46065512 103.0
0.46689415 69.0
0.47313318 58.0
0.4793722 51.0
0.4856112 42.0
0.49185023 33.0
0.49808925 25.0
0.5043283 26.0
0.5105673 17.0
0.51680636 19.0
0.52304536 9.0
0.52928436 18.0
0.5355234 7.0
0.5417624 10.0
0.54800147 8.0
0.55424047 0.0
0.5604795 8.0
0.5667185 3.0
0.5729576 3.0
0.58 0.0
}{\sgapneg}

\pgfplotstableread{
sim dist
0.3989706 0.0
0.41946614 4.0
0.43996167 8.0
0.4604572 1.0
0.4809527 8.0
0.5014483 20.0
0.5219438 30.0
0.5424393 24.0
0.5629348 36.0
0.58343035 42.0
0.6039259 34.0
0.6244214 68.0
0.64491695 46.0
0.6654125 44.0
0.685908 44.0
0.70640355 26.0
0.7268991 48.0
0.74739456 24.0
0.7678901 14.0
0.7883856 4.0
0.80888116 10.0
0.8293767 8.0
0.84 0.0
}{\sappos}

\pgfplotstableread{
sim dist
0.40 0.0
0.4539408 134.0
0.46501255 81.0
0.47608426 90.0
0.48715597 70.0
0.49822772 42.0
0.50929946 48.0
0.5203712 39.0
0.5314429 24.0
0.5425146 24.0
0.55358636 15.0
0.56465805 4.0
0.5757298 2.0
0.5868015 14.0
0.5978733 1.0
0.608945 8.0
0.6200167 1.0
0.63108844 0.0
0.6421602 0.0
0.65323186 2.0
0.6643036 1.0
0.67 0.0
}{\sapneg}


==> data/tauq_hist.tex <==
\pgfplotstableread[col sep=space]{
tau msap gsap rsk
0.4025 0.1275 0.0857 0.0901
0.4075 0.1429 0.0659 0.1055
0.4125 0.1407 0.0857 0.1736
0.4175 0.1231 0.1099 0.1341
0.4225 0.1473 0.0769 0.1583
0.4275 0.2000 0.1341 0.1714
0.4325 0.1561 0.1143 0.2000
0.4375 0.1956 0.1275 0.1671
0.4425 0.2308 0.1253 0.2154
0.4475 0.2374 0.1275 0.2594
0.4525 0.3121 0.1385 0.2704
0.4575 0.2857 0.1407 0.2660
0.4625 0.3341 0.1341 0.3341
0.4675 0.4000 0.1802 0.3561
0.4725 0.4000 0.1846 0.4044
0.4775 0.4308 0.1868 0.4946
0.4825 0.5143 0.1868 0.6330
0.4875 0.6133 0.2440 0.6572
0.4925 0.7188 0.2813 0.7627
0.4975 0.8748 0.3143 0.8199
0.5025 0.9847 0.2352 1.0287
0.5075 1.0045 0.3319 1.1760
0.5125 1.3122 0.4660 1.2265
0.5175 1.5364 0.4484 1.5057
0.5225 1.5123 0.5759 1.6793
0.5275 1.8376 0.6902 1.7650
0.5325 2.1277 0.7891 1.9057
0.5375 2.2706 0.8704 2.0134
0.5425 2.4728 1.1342 2.3827
0.5475 2.5629 1.3320 2.4178
0.5525 2.8553 1.5342 2.7300
0.5575 3.0926 1.8002 2.8662
0.5625 3.1872 2.1585 3.0047
0.5675 3.2971 2.4464 3.2421
0.5725 3.7191 2.6201 3.4399
0.5775 3.7037 3.1146 3.5498
0.5825 3.8773 2.9937 3.6817
0.5875 3.9455 3.6949 3.5037
0.5925 3.8400 3.7850 3.8466
0.5975 4.0136 3.9235 3.8158
0.6025 4.1697 3.9565 4.2202
0.6075 4.2334 4.2774 4.0576
0.6125 4.1719 4.7632 4.1125
0.6175 4.2224 4.6599 4.0026
0.6225 4.3543 4.7851 4.2356
0.6275 4.0532 4.9632 4.1851
0.6325 4.2950 5.0577 4.3939
0.6375 4.0796 4.7676 4.2730
0.6425 3.7938 4.7016 4.1807
0.6475 4.0862 4.7478 3.9301
0.6525 3.9015 4.5983 3.9894
0.6575 3.8202 4.6291 3.8422
0.6625 3.8642 4.4005 3.8488
0.6675 3.7015 4.3543 3.7762
0.6725 3.5103 4.1851 3.5498
0.6775 3.6048 4.2576 3.7477
0.6825 3.3828 4.2906 3.5850
0.6875 3.4553 4.2180 3.3740
0.6925 3.2575 4.0532 3.2047
0.6975 3.0487 3.8246 3.1058
0.7025 3.0575 3.6312 3.2421
0.7075 2.8091 3.4026 3.0289
0.7125 2.7827 3.4136 2.9344
0.7175 2.7300 3.0707 2.8069
0.7225 2.5563 3.0817 2.6860
0.7275 2.5409 2.9740 2.5563
0.7325 2.5080 2.7673 2.5365
0.7375 2.2002 2.7541 2.2134
0.7425 2.0706 2.6706 2.1914
0.7475 2.1497 2.4003 2.1211
0.7525 1.9607 2.3014 2.0442
0.7575 1.8925 2.2156 1.9804
0.7625 1.7694 2.1123 1.8288
0.7675 1.7694 2.1123 1.8486
0.7725 1.5298 1.9145 1.7189
0.7775 1.4771 1.8200 1.5980
0.7825 1.3782 1.6991 1.4595
0.7875 1.4067 1.7518 1.3628
0.7925 1.3122 1.4529 1.3078
0.7975 1.1496 1.4485 1.1869
}\tauqsop

\pgfplotstableread[col sep=space]{
tau msap gsap rsk
0.4025 0.3127 0.0680 0.2719
0.4075 0.3399 0.0952 0.2447
0.4125 0.2855 0.1223 0.2175
0.4175 0.4486 0.1359 0.2039
0.4225 0.3806 0.1767 0.2991
0.4275 0.4350 0.1631 0.2447
0.4325 0.5030 0.1767 0.2719
0.4375 0.5166 0.2991 0.6117
0.4425 0.7205 0.2447 0.4894
0.4475 0.6117 0.2855 0.4350
0.4525 0.7749 0.2719 0.5710
0.4575 0.8972 0.2175 0.6389
0.4625 0.9108 0.4078 0.6797
0.4675 0.8972 0.5030 0.7069
0.4725 1.0196 0.3127 0.8836
0.4775 1.4954 0.4350 0.9924
0.4825 1.6313 0.5574 1.2643
0.4875 1.7673 0.6933 1.2643
0.4925 1.9576 0.7613 1.7537
0.4975 2.1615 0.7477 1.8624
0.5025 2.3790 0.8293 1.7945
0.5075 2.6645 0.9924 2.0256
0.5125 2.8276 1.3051 2.1343
0.5175 2.6237 1.4002 2.5557
0.5225 3.2355 1.6585 3.1947
0.5275 3.5345 1.6721 2.3110
0.5325 3.9016 2.3382 3.1675
0.5375 4.5405 2.5014 3.4530
0.5425 4.3774 2.7868 3.8608
0.5475 4.9076 3.4666 3.9016
0.5525 4.9212 3.2219 3.9695
0.5575 5.3562 4.4861 4.4997
0.5625 5.3290 4.9076 4.7580
0.5675 5.5193 5.0979 4.9483
0.5725 5.8592 5.5329 5.4649
0.5775 5.0979 5.4377 5.2882
0.5825 5.5057 6.0903 5.3834
0.5875 5.7368 6.2534 6.1446
0.5925 5.6417 6.6204 5.6145
0.5975 5.6552 7.3681 6.2806
0.6025 5.2066 6.8787 5.4921
0.6075 5.3834 6.7972 5.5873
0.6125 5.3970 7.2458 6.0223
0.6175 5.3290 6.5389 5.7232
0.6225 4.5133 7.2050 5.3154
0.6275 4.5677 7.3681 5.2882
0.6325 4.4997 6.9059 5.0843
0.6375 4.0511 6.4573 4.9755
0.6425 3.8880 5.9407 4.3230
0.6475 3.3850 5.5737 4.2550
0.6525 3.5753 5.0435 4.0375
0.6575 3.6297 4.6493 4.3638
0.6625 3.2626 4.4182 3.4394
0.6675 3.1675 4.2414 3.2490
0.6725 2.3654 3.8744 3.2083
0.6775 2.3246 3.2762 3.3306
0.6825 2.7053 3.1267 3.0315
0.6875 2.3790 2.6917 2.5150
0.6925 2.1343 2.5285 2.7461
0.6975 1.7945 2.2974 2.2431
0.7025 1.8760 2.0799 1.7945
0.7075 1.4410 1.7537 1.8352
0.7125 1.4138 1.5090 1.5362
0.7175 1.1011 1.1691 1.3594
0.7225 0.9108 0.9924 1.1827
0.7275 0.9924 0.6253 1.2915
0.7325 0.8564 0.9244 1.1419
0.7375 0.6389 0.6933 0.8564
0.7425 0.8564 0.7749 0.8836
0.7475 0.5030 0.6797 0.8564
0.7525 0.3942 0.3670 0.8428
0.7575 0.5302 0.3263 0.5574
0.7625 0.4214 0.3399 0.4486
0.7675 0.5166 0.3942 0.5166
0.7725 0.3535 0.1223 0.4758
0.7775 0.3127 0.0952 0.3399
0.7825 0.2855 0.2311 0.2447
0.7875 0.2583 0.2311 0.3263
0.7925 0.1631 0.0680 0.1767
0.7975 0.0816 0.1631 0.2175
}\tauqinat

